A Machine Learning Approach to Improving Timing Consistency between Global Route and Detailed Route

Due to the unavailability of routing information in design stages prior to detailed routing (DR), the tasks of timing prediction and optimization pose major challenges. Inaccurate timing prediction wastes design effort, hurts circuit performance, and may lead to design failure. This work focuses on timing prediction after clock tree synthesis and placement legalization, which is the earliest opportunity to time and optimize a "complete" netlist. The paper first documents that having "oracle knowledge" of the final post-DR parasitics enables post-global routing (GR) optimization to produce improved final timing outcomes. To bridge the gap between GR-based parasitic and timing estimation and post-DR results during post-GR optimization, machine learning (ML)-based models are proposed, including the use of features for macro blockages for accurate predictions for designs with macros. Based on a set of experimental evaluations, it is demonstrated that these models show higher accuracy than GR-based timing estimation. When used during post-GR optimization, the ML-based models show demonstrable improvements in post-DR circuit performance. The methodology is applied to two different tool flows - OpenROAD and a commercial tool flow - and results on 45nm bulk and 12nm FinFET enablements show improvements in post-DR slack metrics without increasing congestion. The models are demonstrated to be generalizable to designs generated under different clock period constraints and are robust to training data with small levels of noise.

==> coverletter.tex <==
\noindent\textbf{Cover Letter}
\vspace{1.0em}


\noindent
Dear Editor,

\noindent We are submitting this paper for potential publication in ACM TODAES. This manuscript is an enhancement of the following paper:
\vspace{1.0em}

\noindent V. A. Chhabria, W. Jiang, A. B. Kahng, and S. Sapatnekar, “From Global Route to Detailed Route: ML for Fast and Accurate Wire Parasitics and Timing Prediction,” \textit{Proceedings of ACM/IEEE Workshop on Machine Learning for CAD (MLCAD)}, 2022
\vspace{1.0em}

\noindent The previous paper proposed an initial framework for machine-learning-based models for parasitics and timing estimation, and a flow that optimizes design based on ML prediction. These models use the features extracted after global routing to predict the timing of post-detailed routing more accurately, and the design is optimized based on our prediction after global routing, which improves the quality of the final results in several metrics.

\noindent
In this expanded version, we add several significant enhancements to the preliminary version of the work:
\begin{itemize}
\item We consider realistic designs that contain macros within the design.  The presence of macros significantly complicates the task of timing prediction as it introduces routing blockages that reduce routability in the neighborhood of the macro.  This necessitates routing detours, which influence the interconnect delay and parasitics. In this submission, we motivate this problem and quantify its impact, and create an ML modeling methodology that includes features that incorporate the impact of routing blockages.  We demonstrate that this approach provides significantly better results than our preliminary work, and than a traditional timing prediction method.
\item While the previous approach focused on bulk technology nodes, we have conducted experiments on applying the approach on a FinFET technology node, which has more stringent limitations (e.g., unidirectional routing in lower metal layers) and demonstrate that our approach works for such designs.
\item We show that the methodology can be used across tool flows, applying it not only for the OpenROAD flow (as in the preliminary version) but also a commercial tool flow. 
\item We test the sensitivity of the ML model to different clock constraints, including applying it to predict the timing for unseen configurations for the circuit.  Furthermore, since the results of design tools are often noisy, the training data could have a certain amount of noise. We test the robustness of the model to training noise and show that it has a level of robustness that can tolerate noise in the data used to train the model.
\end{itemize}
In addition, we have added more detailed explanations and motivating graphs throughout the manuscript. The blue text in the paper reflects the changes from the preliminary conference version (in addition, the tables and figures in the results section are entirely new or significantly updated).  We believe that, collectively, these changes meet the threshold of a 30\% differential between the preliminary work and a journal submission.\\

% \noindent ~\redFN{Perhaps better to create a bullet point list of differences?} The preliminary results were shown on the models without consideration of macros in the design. The macro block reduces the routability of its surrounding space, which influences the interconnect delay and parasitics~\redFN{Need a number by how much wires can detour due to blockages?}. In this submission, we introduce the features for routing blockage due to macros in the model training.
% \vspace{1.0em}

% \noindent In addition to the previous paper that implements all designs with OpenROAD in two opensource technologies, NG45 and Skywater130, we extend it by applying the proposed ML-based flow in commercial tools and implementing designs in one commercial technology, GF12. 
% \vspace{1.0em}

% \noindent The results section has been strengthened to incorporate the additional observations in larger designs and GF12 technology, test the model sensitivity to different clock constraints and test the model robustness to noise. Overall, the results section justifies the use of new feature to increase the prediction accuracy and improve the design quality in post-detailed routing~\redFN{Difficult to say this unless we show comparisons to MLCAD22. We need to have our results support this so we need to state the importance of macros to the overall metrics} . In the ultra-scaled technology, more benefits from the proposed methods are observed. Moreover, our methodology is not only applicable to the opensource tool but also to the commercial tool.

\noindent
Sincerely,\\
Wenjing Jiang\\
(on behalf of co-authors Vidya A. Chhabria, Andrew B. Kahng, and Sachin S. Sapatnekar)

==> misc/customize.tex <==
\usepackage{float} 
\usepackage{tabularx}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{hhline}
\usepackage{silence}
\usepackage{graphicx}
\usepackage{multirow} 
\usepackage{graphicx}
\usepackage{multirow}
\usepackage[english]{babel}
\usepackage{booktabs}
\usepackage{array}
\usepackage{paralist}
\usepackage{threeparttable}
\usepackage{lipsum}
\usepackage{flushend}
\usepackage{cuted}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{color}
\usepackage{psfrag}
\usepackage{epsfig}
\usepackage{multicol}
\usepackage{color}
\usepackage{fancybox}
\usepackage{subfigure}
\usepackage{cite}
\usepackage{theorem}
\usepackage{url}
\usepackage[table]{xcolor}
\usepackage{epstopdf}
\usepackage[normalem]{ulem}
\usepackage{siunitx}
\usepackage{rotating}
\usepackage{adjustbox}

%\usepackage{biblatex} 
%\usepackage[backend=biber]{biblatex}
%\usepackage[style=apa,sortcites=true,sorting=nyt,backend=biber]{biblatex}
%\usepackage{subcaption}
\usepackage[justification=centering,font=small,labelfont=bf]{caption}
% \usepackage[font=small,labelfont=bf]{caption}
\usepackage{silence}
\WarningFilter{caption}{Unsupported document class}
\usepackage{enumitem}
%\usepackage{widetext}
%\usepackage{paralist}
%\usepackage[none]{hyphenat}
\definecolor{gray1}{gray}{0.90}
\definecolor{gray2}{gray}{0.98}
\definecolor{light-gray}{gray}{0.95}
\def\bibfont{\scriptsize}
%Adds extra padding to the table cells
\setlength\extrarowheight{2pt}

\newcommand{\ignore}[1]{}
\newcommand{\redHL}[1]{\textcolor{red}{#1}}
\newcommand{\blueHL}[1]{{\textcolor{blue}{#1}}}
\newcommand{\greenHL}[1]{\textcolor{green}{#1}}
\newcommand{\grayHL}[1]{\textcolor{gray}{#1}}
\newcommand{\blackHL}[1]{\textcolor{black}{#1}}
\newcommand{\redfn}[1]{\redHL{\footnote{\redHL{#1}}}
\newcommand{\Alter}[2]{\sout{#1}\redHL{#2}}
\newcommand{\txtoverline}[1]{$\overline{\mbox{{#1}}}$}
\newcommand{\TMR}{\mbox{TMR}}
\newcommand{\sTMR}{\scriptsize{\mbox{TMR}}}
%\newcommand{\Deff}{D_{\mbox{\tiny \em eff}}}
%\newcommand{\Deffn}{D_{\mbox{\tiny \em eff,n}}}
%\newcommand{\Deffg}{D_{\mbox{\tiny \em eff,g}}}
%\newcommand{\Zeff}{Z^\star_{\mbox{\tiny \em eff}}}
%\newcommand{\Javg}{J_{\mbox{\tiny \em avg}}}
%\newcommand{\Jeff}{J_{\mbox{\tiny \em eff}}}
%\newcommand{\Jrms}{J_{\mbox{\tiny \em rms}}}
%\newcommand{\Jflux}{J_{\mbox{\tiny \em flux}}}
%\newcommand{\vivekeq}[1]{\mbox{\tiny {\em #1}}}
%\newcommand{\Tlife}{T_{\mbox{\tiny \em life}}}
%\newcommand{\Ieff}{I_{\mbox{\tiny \em eff}}}
%\newcommand{\Irise}{I_{\mbox{\tiny \em rise}}}
%\newcommand{\Jpavg}{J_{\vivekeq{avg}}^+}
%\newcommand{\Jnavg}{J_{\vivekeq{avg}}^-}
%\newcommand{\Jbavg}{J_{\vivekeq{avg}}^{\vivekeq{blue}}}
%\newcommand{\Jgavg}{J_{\vivekeq{avg}}^{\vivekeq{green}}}
%\newcommand{\nuc}{t_{\mbox{\scriptsize \it nuc}}}
%\newcommand{\nucs}{t_{\mbox{\scriptsize \it nuc--SI}}}
%\newcommand{\nucf}{t_{\mbox{\scriptsize \it nuc--F}}}
%\newcommand{\tlife}{t_{\mbox{\scriptsize \it life}}}
%\newcommand{\Mx}{\mbox{M}_{\mbox{\scriptsize x}}}
%\newcommand{\Mxp}{\mbox{M}_{\mbox{\scriptsize x+1}}}
%\pagestyle{plain}
%\renewcommand{\bibfont}{\tiny}
\usepackage{tikz}
%\usetikzlibrary{tikzmark}
%\usetikzlibrary{shapes,arrows}
%\renewcommand{\baselinestretch}{0.93}
%\selectcolormodel{gray}

==> tbl/macro-impact-on-DR.tex <==
\begin{table}
\centering
\caption{Macro feature impact on post-DR slacks.}
\label{tbl:macro-impact-on-DR}
\resizebox{0.6\linewidth}{!}{\begin{tabular}{|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\textbf{Design}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{CLK}\\\textbf{(ns)}\end{tabular}} & \multirow{2}{*}{\textbf{Tech}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Die size}\\\textbf{(mm\textsuperscript{2})}\end{tabular}} & \multicolumn{2}{c|}{\textbf{Post-DR TNS for detour sets (ns)}}  \\ 
\cline{5-6}
                                 &                                                                                      &                                &                                                                                                              & \textbf{ML~based} & \textbf{Old ML~based}                       \\ 
\hline
\multirow{3}{*}{swerv\_wrapper}  & \multirow{3}{*}{2.5}                                                                 & \multirow{9}{*}{45nm}          & 1.20x1.09                                                                                                    & 0.00              & 0.00                                        \\ 
\cline{4-6}
                                 &                                                                                      &                                & 1.36x1.20                                                                                                    & -0.18             & -0.21                                       \\ 
\cline{4-6}
                                 &                                                                                      &                                & 1.55x1.34                                                                                                    & -0.51             & -0.56                                       \\ 
\cline{1-2}\cline{4-6}
\multirow{3}{*}{bp\_fe}          & \multirow{3}{*}{2.2}                                                                 &                                & 0.78x0.63                                                                                                    & -1.39             & -1.44                                       \\ 
\cline{4-6}
                                 &                                                                                      &                                & 0.84x0.68                                                                                                    & 0.00              & 0.00                                        \\ 
\cline{4-6}
                                 &                                                                                      &                                & 0.99x0.79                                                                                                    & 0.00              & 0.00                                        \\ 
\cline{1-2}\cline{4-6}
\multirow{3}{*}{bp\_be}          & \multirow{3}{*}{2.8}                                                                 &                                & 0.75x0.75                                                                                                    & -6.50             & -7.10                                       \\ 
\cline{4-6}
                                 &                                                                                      &                                & 0.79x0.78                                                                                                    & -6.75             & -6.83                                       \\ 
\cline{4-6}
                                 &                                                                                      &                                & 0.98x0.92                                                                                                    & -2.10             & -2.63                                       \\ 
\hline
\multirow{3}{*}{swerv\_wrapper}  & \multirow{3}{*}{1.2}                                                                 & \multirow{6}{*}{12nm}          & 0.64x0.48                                                                                                    & -0.18             & -0.89                                       \\ 
\cline{4-6}
                                 &                                                                                      &                                & 0.70x0.54                                                                                                    & -2.80             & -2.93                                       \\ 
\cline{4-6}
                                 &                                                                                      &                                & 0.80x0.64                                                                                                    & -10.07            & -12.39                                      \\ 
\cline{1-2}\cline{4-6}
\multirow{3}{*}{coyote}          & \multirow{3}{*}{3.2}                                                                 &                                & 0.66x0.66                                                                                                    & 0.00              & 0.00                                        \\ 
\cline{4-6}
                                 &                                                                                      &                                & 0.75x0.75                                                                                                    & -0.11             & -0.19                                       \\ 
\cline{4-6}
                                 &                                                                                      &                                & 0.85x0.85                                                                                                    & -0.04             & -0.16                                       \\
\hline
\end{tabular}}
\end{table}

==> tbl/sink-based-accuracy.tex <==
\begin{table}
\centering
\caption{\blueHL{Evaluation of the ML models using mean, maximum, and standard deviation of the absolute \%error as metrics.}}
\label{tbl:ml-sink-accuracy}
\resizebox{\linewidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
% \textbf{Tool}          & \textbf{Designs}                & \begin{tabular}[c]{@{}c@{}}\textbf{Clock}\\\textbf{period}\end{tabular} & \textbf{Tech}         & \textbf{Metrics}  & \begin{tabular}[c]{@{}c@{}}\textbf{ML wire}\\\textbf{delay}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{GR wire}\\\textbf{delay}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{ML wire}\\\textbf{slew}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{GR wire}\\\textbf{slew}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{ML path}\\\textbf{slack}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{GR path}\\\textbf{slack}\end{tabular}  \\ 
\textbf{Tool}          & \textbf{Designs}                & \textbf{Clock}  & \textbf{Technology}         & \textbf{Metrics}   & \multicolumn{2}{c|}{\bf Wire delay} & \multicolumn{2}{c|}{\bf Slew} & \multicolumn{2}{c|}{\bf Path delay}  \\ \cline{6-11}
                        &                                 & \textbf{period} & \textbf{node}              &                    &
\textbf{ML-based} & \textbf{GR-based} & \textbf{ML-based} & \textbf{GR-based} & \textbf{ML-based} & \textbf{GR-based} \\               
\hline
\multirow{15}{*}{\rotatebox{90}{OpenROAD}}   & \multirow{3}{*}{swerv\_wrapper} & \multirow{3}{*}{2.5ns}                                                  & \multirow{9}{*}{45nm} & Mean \%error      & 0.84\%                                                                   & 4.27\%                                                                   & 0.04\%                                                                  & 0.20\%                                                                  & 0.34\%                                                                   & 1.48\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 115.19\%                                                                 & 149.41\%                                                                 & 19.81\%                                                                 & 40.63\%                                                                 & 4.62\%                                                                   & 7.54\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 2.78\%                                                                   & 7.28\%                                                                   & 0.34\%                                                                  & 1.22\%                                                                  & 0.30\%                                                                   & 0.69\%                                                                    \\ 
\cline{2-3}\cline{5-11}
                       & \multirow{3}{*}{bp\_fe}         & \multirow{3}{*}{2.2ns}                                                  &                       & Mean \%error      & 0.64\%                                                                   & 3.63\%                                                                   & 0.04\%                                                                  & 0.24\%                                                                  & 0.65\%                                                                   & 0.69\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & \textcolor{red}{19.14\%}                                                 & 15.68\%                                                                  & 4.42\%                                                                  & 5.83\%                                                                  & 1.91\%                                                                   & 2.47\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 0.91\%                                                                   & 4.65\%                                                                   & 0.13\%                                                                  & 0.98\%                                                                  & 0.41\%                                                                   & 0.52\%                                                                    \\ 
\cline{2-3}\cline{5-11}
                       & \multirow{3}{*}{bp\_be}         & \multirow{3}{*}{2.8ns}                                                  &                       & Mean \%error      & 2.16\%                                                                   & 3.00\%                                                                   & 0.07\%                                                                  & 0.12\%                                                                  & 0.63\%                                                                   & 0.80\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 34.58\%                                                                  & 55.64\%                                                                  & 9.15\%                                                                  & 10.45\%                                                                 & 2.21\%                                                                   & 2.57\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 3.42\%                                                                   & 3.88\%                                                                   & 0.25\%                                                                  & 0.38\%                                                                  & \textcolor{red}{0.45\%}                                                  & 0.34\%                                                                    \\ 
\cline{2-11}
                       & \multirow{3}{*}{swerv\_wrapper} & \multirow{3}{*}{1.2ns}                                                 & \multirow{6}{*}{12nm} & Mean \%error      & 0.87\%                                                                   & 4.26\%                                                                   & 0.04\%                                                                  & 0.70\%                                                                  & 1.15\%                                                                   & 5.75\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 22.80\%                                                                  & 44.95\%                                                                  & 29.81\%                                                                 & 71.75\%                                                                 & 7.61\%                                                                   & 14.91\%                                                                   \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 0.93\%                                                                   & 5.76\%                                                                   & 0.17\%                                                                  & 3.85\%                                                                  & 1.26\%                                                                   & 4.77\%                                                                    \\ 
\cline{2-3}\cline{5-11}
                       & \multirow{3}{*}{coyote}         & \multirow{3}{*}{3.2ns}                                                 &                       & Mean \%error      & 0.60\%                                                                   & 3.47\%                                                                   & 0.22\%                                                                  & 1.97\%                                                                  & 1.09\%                                                                   & 1.23\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 26.58\%                                                                  & 39.65\%                                                                  & 40.13\%                                                                 & 51.34\%                                                                 & 2.65\%                                                                   & 7.73\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 0.88\%                                                                   & 4.73\%                                                                   & 0.62\%                                                                  & 4.51\%                                                                  & 0.27\%                                                                   & 1.51\%                                                                    \\ 
\hline
\multirow{15}{*}{\rotatebox{90}{Commercial tool}} & \multirow{3}{*}{swerv\_wrapper} & \multirow{3}{*}{2.2ns}                                                  & \multirow{9}{*}{45nm} & Mean \%error      & 7.21\%                                                                   & 29.80\%                                                                  & 0.24\%                                                                  & 1.46\%                                                                  & 0.35\%                                                                   & 1.00\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 63.59\%                                                                  & 70.56\%                                                                  & 9.14\%                                                                  & 50.93\%                                                                 & 5.49\%                                                                   & 5.94\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 6.50\%                                                                   & 11.56\%                                                                  & 0.71\%                                                                  & 5.28\%                                                                  & 0.53\%                                                                   & 0.60\%                                                                    \\ 
\cline{2-3}\cline{5-11}
                       & \multirow{3}{*}{bp\_fe}         & \multirow{3}{*}{1.6ns}                                                  &                       & Mean \%error      & 5.88\%                                                                   & 24.41\%                                                                  & 0.36\%                                                                  & 3.73\%                                                                  & 0.54\%                                                                   & 1.64\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 43.79\%                                                                  & 51.07\%                                                                  & 6.08\%                                                                  & 37.84\%                                                                 & 4.81\%                                                                   & 7.05\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 4.96\%                                                                   & 9.26\%                                                                   & 0.79\%                                                                  & 8.83\%                                                                  & 0.46\%                                                                   & 0.67\%                                                                    \\ 
\cline{2-3}\cline{5-11}
                       & \multirow{3}{*}{bp\_be}         & \multirow{3}{*}{2.0ns}                                                  &                       & Mean \%error      & 6.09\%                                                                   & 25.84\%                                                                  & 0.36\%                                                                  & 3.04\%                                                                  & 0.60\%                                                                   & 1.65\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 57.99\%                                                                  & 56.00\%                                                                  & 19.30\%                                                                 & 99.94\%                                                                 & 5.08\%                                                                   & 6.28\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 5.46\%                                                                   & 9.29\%                                                                   & 0.83\%                                                                  & 7.84\%                                                                  & 0.47\%                                                                   & 0.50\%                                                                    \\ 
\cline{2-11}
                       & \multirow{3}{*}{swerv\_wrapper} & \multirow{3}{*}{1.0ns}                                                 & \multirow{6}{*}{12nm} & Mean \%error      & 6.24\%                                                                   & 12.30\%                                                                  & 0.36\%                                                                  & 0.85\%                                                                  & 3.52\%                                                                   & 5.98\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 36.47\%                                                                  & 56.30\%                                                                  & 26.26\%                                                                 & 79.14\%                                                                 & 8.28\%                                                                   & 13.69\%                                                                   \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 1.27\%                                                                   & 2.78\%                                                                   & 0.95\%                                                                  & 2.78\%                                                                  & 2.29\%                                                                   & 3.24\%                                                                    \\ 
\cline{2-3}\cline{5-11}
                       & \multirow{3}{*}{coyote}         & \multirow{3}{*}{3.2ns}                                                 &                       & Mean \%error      & 5.22\%                                                                   & 15.42\%                                                                  & 3.68\%                                                                  & 11.75\%                                                                 & 2.22\%                                                                   & 4.67\%                                                                    \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Max \%error       & 83.62\%                                                                  & 98.70\%                                                                  & 59.35\%                                                                 & 93.02\%                                                                 & 7.36\%                                                                   & 10.85\%                                                                   \\ 
\cline{5-11}
                       &                                 &                                                                         &                       & Std. dev. \%error & 1.05\%                                                                   & 2.99\%                                                                   & 0.88\%                                                                  & 2.86\%                                                                  & 1.74\%                                                                   & 2.87\%                                                                    \\
\hline
\end{tabular}}
\end{table}

==> tbl/tbl4-alt.tex <==
\begin{table}
\centering
\caption{\blueHL{Evaluation of the ML models using mean, maximum, and standard deviation of the absolute \%error as metrics.}}
\label{tbl:ml-sink-accuracy}
\begin{adjustbox}{angle=90}
\resizebox{\textheight}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\textbf{Tool}          & \textbf{Designs}                & \textbf{Clock}  & \textbf{Technology}        & \multicolumn{6}{c|}{\bf Wire delay} & \multicolumn{6}{c|}{\bf Slew} & \multicolumn{6}{c|}{\bf Path delay}  \\ \cline{5-22}
                        &                                 & \textbf{period} & \textbf{node}              &
\multicolumn{3}{c|}{\textbf{ML-based}} & \multicolumn{3}{c|}{\textbf{GR-based}} & \multicolumn{3}{c|}{\textbf{ML-based}} & \multicolumn{3}{c|}{\textbf{GR-based}} & \multicolumn{3}{c|}{\textbf{ML-based}} & \multicolumn{3}{c|}{\textbf{GR-based}} \\   \cline{5-22}  
& & & & Mean & Max & Stdev. & Mean & Max & Stdev. & Mean & Max & Stdev. & Mean & Max & Stdev. & Mean & Max & Stdev. & Mean & Max & Stdev. \\ \hline
\multirow{3}{*}{OpenROAD}   & swerv\_wrapper & 2.5ns                                                  & \multirow{3}{*}{45nm} & 0.84\%  & 115.19\% & 2.78\%                                                                & 4.27\% &149.41\% & 7.28\%                                                                & 0.04\% & 19.81\% & 0.34\%                                                                 & 0.20\% & 40.63\% & 1.22\%                                                                 & 0.34\% & 4.62\% & 0.30\%                                                                  & 1.48\% & 7.54\% & 0.69\%                                                                   \\ 
\cline{2-3}\cline{5-22}
                       & bp\_fe         & 2.2ns & & & & & & & & & & & & & & & & & & & \\ \cline{2-3}\cline{5-22}
                       & bp\_fe         & 2.8ns & & & & & & & & & & & & & & & & & & & \\ \hline
\end{tabular}
}
\end{adjustbox}
\end{table}
